Fast and Scalable Estimator for Sparse and Unit-Rank Higher-Order Regression Models

Because tensor data appear more and more frequently in various scientific researches and real-world applications, analyzing the relationship between tensor features and the univariate outcome becomes an elementary task in many fields. To solve this task, we propose \underline{Fa}st \underline{S}parse \underline{T}ensor \underline{R}egression model (FasTR) based on so-called unit-rank CANDECOMP/PARAFAC decomposition. FasTR first decomposes the tensor coefficient into component vectors and then estimates each vector with $\ell_1$ regularized regression. Because of the independence of component vectors, FasTR is able to solve in a parallel way and the time complexity is proved to be superior to previous models. We evaluate the performance of FasTR on several simulated datasets and a real-world fMRI dataset. Experiment results show that, compared with four baseline models, in every case, FasTR can compute a better solution within less time.

==> macros.tex <==
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{epsfig}

\def\Q{{\mathbb Q}}        % rationals
\def\Z{{\mathbb Z}}        % integers
\def\N{{\mathbb N}}        % naturals
\def\R{{\mathbb R}}        % reals
\def\C{{\mathbb C}} 	   % complex
\def\Rn{{\R^{n}}}          % product of n copies of reals
\def\Cf{{\mathbf C}}	   % continuous functions on (.)

\def\P{{\mathbb P}}        % probability
\def\E{{\mathbb E}}        % expectation 
\def\1{{\mathbf 1}}        % indicator
\def\var{{\mathop{\mathbf Var}}}    % variance

\def\done{\hfill\rule{2mm}{2mm}}

\def\borel{{\cal B}}    % borel sigmal field
\def\G{{\cal G}}        % some sigma field
\def\F{{\cal F}}        % some sigma field
\def\H{{\cal H}}        % some sigma field

\def\L{{\mathbf L}}     % L, as in L^2

\def\ascv{\stackrel{\scriptscriptstyle a.s.}{\longrightarrow}}     % almost sure convergnece
\def\pcv{\stackrel{\scriptscriptstyle \P}{\longrightarrow}}        % convergence in P
\def\ltcv{\stackrel{\scriptscriptstyle\L^2}{\longrightarrow}}      % L2 convergence
\def\lpcv{\stackrel{\scriptscriptstyle\L^p}{\longrightarrow}}      % Lp convergence
\def\dcv{\stackrel{\scriptscriptstyle d}{\longrightarrow}}         % convergence in d
\def\deq{\stackrel{\scriptscriptstyle d}{=}}			   % equal in d
\def\toinf{\to \infty}

\def\ci{\perp\!\!\!\perp}  % conditional independence

% the header/lecture structure...borrowed from alistair sinclair's cs270 format
\newcommand{\topic}[4]{
   \pagestyle{myheadings}
   \thispagestyle{plain}
   \newpage
   \setcounter{page}{1}
   \noindent
   \begin{center}
   \framebox{
      \vbox{\vspace{2mm}
    \hbox to 6.28in { {\bf MATH 7360~Probability Theory I
                        \hfill Fall 2013} }
       \vspace{4mm}
       \hbox to 6.28in { {\Large \hfill Lecture #1: #2 \hfill} }
       \vspace{2mm}
			\hbox to 6.28in { {\it #4}\hfill}
       \hbox to 6.28in { {\it Lecturer:} Tai Melcher \hfill {\it Scribe:} #3}
      \vspace{2mm}}
   }
   \end{center}
   \markboth{Topic: #1}{Topic: #1}
   \vspace*{4mm}
}
       %\hbox to 5.90in { \hfill {\it Scribe: #3} }


%\newtheorem{theorem}{Theorem}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{claim}[theorem]{Claim}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{definition}[theorem]{Definition}
%\newenvironment{proof}{{\bf Proof:}}{\hfill\rule{2mm}{2mm}}
\newenvironment{proofsketch}{{\bf Proof Sketch:}}{\hfill\rule{2mm}{2mm}}
\newcommand{\fig}[3]{
      \vspace{#2}
      \begin{center}
      Figure #1:~#3
      \end{center}
}
%\newtheorem{exercise}[theorem]{Exercise}
%\newtheorem{example}[theorem]{Example}

%some things we'll never understand....alas




==> preamble.tex <==
\usepackage{multirow}
%\pagenumbering{roman}


%for caption font
\usepackage[font=scriptsize]{caption}

\usepackage{wrapfig}


\newcommand{\titleName}{}


% for utility 
\newcommand{\ie}{i.e., }
\newcommand{\eg}{e.g., }

% For math
\usepackage{math-Header}

\newcommand{\eref}[1]{Eq.~(\ref{#1})} 
\newcommand{\rref}[1]{Theorem~(\ref{#1})} 
\newcommand{\iref}[1]{Inequality~(\ref{#1})} 
\newcommand{\lref}[1]{Lemma~(\ref{#1})} 
\newcommand{\cref}[1]{Condition~(\ref{#1})} 
\newcommand{\dref}[1]{Definition~(\ref{#1})} 
\newcommand{\coref}[1]{Corollary~(\ref{#1})}
\newcommand{\secref}[1]{Section~\ref{#1}} 
\newcommand{\figref}[1]{Figure~(\ref{#1})} 
\newcommand{\tabref}[1]{Table~(\ref{#1})} 




\include{macros}



% For figures
\usepackage{subfigure} 

% For algorithms
\usepackage{algorithm}
\usepackage{algorithmic}
%\newcommand{\theHalgorithm}{\arabic{algorithm}}



%-------------------------------------------------
%%% Tags below controls certain sections to appear or not 
\newboolean{doShortv}
%\setboolean{doShortv}{true}
\setboolean{doShortv}{false}


\newboolean{doLongv}
\setboolean{doLongv}{true}
%\setboolean{doLongv}{false}


\usepackage{flushend}

\iffalse
%-------------------------------------------------
% For heading spacing 
\usepackage{lipsum}
\usepackage{titlesec}

%\titlespacing{command}{left spacing}{before spacing}{after spacing}[right]
\titlespacing\section{1pt}{2pt plus 1pt minus 1pt}{1pt plus 1pt minus 1pt}
\titlespacing\subsection{0pt}{1pt plus 0pt minus 1pt}{0pt plus 0pt minus 0pt}
\titlespacing\subsubsection{0pt}{0pt plus 0pt minus 1pt}{0pt plus 0pt minus 0pt}
%\titleformat{\paragraph}[runin]{\normalfont\normalsize\bfseries}{\theparagraph}{1em}{}
\titlespacing{\paragraph}{0pt}{0pt}{0pt}[0pt]  
%\parskip 0pt

%\setlength{\textfloatsep}{0pt}

% For table spacing 
\addtolength{\parskip}{-0.5mm}
\usepackage{etoolbox}
\makeatletter
\preto{\@tabular}{\parskip=0pt}
\makeatother


% for equation spacing 
\setlength{\belowdisplayskip}{1pt} \setlength{\belowdisplayshortskip}{0pt}
\setlength{\abovedisplayskip}{1pt} \setlength{\abovedisplayshortskip}{0pt}
\allowdisplaybreaks


% for itemize spacing 
\usepackage{enumitem}
\setlist[itemize]{leftmargin=*}
\fi

% for commenting 
\usepackage{color}
\definecolor{colora}{rgb}{.7, .1, .1}
\newcommand{\fix}[1]{  {\bf \textcolor{colora}{[TO-FIX: #1]}}    }

